Exploring Network-Wide Flow Data with Flowyager

Many network operations, ranging from attack investigation and mitigation to traffic management, require answering network-wide flow queries in seconds. Although flow records are collected at each router, using available traffic capture utilities, querying the resulting datasets from hundreds of routers across sites and over time, remains a significant challenge due to the sheer traffic volume and distributed nature of flow records. In this paper, we investigate how to improve the response time for a priori unknown network-wide queries. We present Flowyager, a system that is built on top of existing traffic capture utilities. Flowyager generates and analyzes tree data structures, that we call Flowtrees, which are succinct summaries of the raw flow data available by capture utilities. Flowtrees are self-adjusted data structures that drastically reduce space and transfer requirements, by 75% to 95%, compared to raw flow records. Flowyager manages the storage and transfers of Flowtrees, supports Flowtree operators, and provides a structured query language for answering flow queries across sites and time periods. By deploying a Flowyager prototype at both a large Internet Exchange Point and a Tier-1 Internet Service Provider, we showcase its capabilities for networks with hundreds of router interfaces. Our results show that the query response time can be reduced by an order of magnitude when compared with alternative data analytics platforms. Thus, Flowyager enables interactive network-wide queries and offers unprecedented drill-down capabilities to, e.g., identify DDoS culprits, pinpoint the involved sites, and determine the length of the attack.

==> Makefile <==
## Fully automated LaTeX Makefile
## (c) Bernhard Ager 2010
## Released under GPLv3 <http://www.gnu.org/licenses/gpl.txt>
##
## This is supposed to work with no (or at most a few) modifications 
## on any LaTeX source directory as a drop in.
## 
## If you have suggestions for or additions to this Makefile, feel free to
## drop me <bernhard@net.t-labs.tu-berlin.de> a mail. I am especially
## interested in further/better auto-conversion rules for picture formats.
##
## Acknowledgements go to Oliver Hohlfeld for proposing a database to track
## auto-generated pictures.
##
## Hard dependencies: GNU make, sed, grep, rm
## Soft dependencies: the tools to convert to the different formats including
## latex, pdflatex, dvips, pstopdf, eps2pdf, fig2dev, inkscape, wmf2eps, ...


## $(MAIN).tex is assumed to be the main latex file
#MAIN=$(basename $(shell grep -Fl '\documentclass' *.tex))
MAIN=paper

## $(TEXFILES) holds all LaTeX source files. Extend wildcard pattern if you
## are holding tex files in subdirectories or adjust to your needs.
TEXFILES=$(wildcard *.tex sections/*.tex)

## $(PICTURES) and $(BIBLIOGRAPHY) try to guess the names of required 
## pictures and bib files. The matching rule is quite primitive and is
## easily confused by clutter in lines with \includegraphics or 
## \bibliography. 
PICTURES=$(shell grep -F '\includegraphics' $(TEXFILES) | \
		grep -v '%.*\\includegraphics' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfimage' $(TEXFILES) | \
		grep -v '%.*\\pgfimage' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfdeclareimage' $(TEXFILES) | \
		grep -v '%.*\\pgfdeclareimage' | sed 's/.*{\([^{}]*\)}.*/\1/')

BIBLIOGRAPHY=$(addsuffix .bib, $(shell grep -F '\bibliography{' $(TEXFILES) | \
	grep -v '%.*\\bibliography' | sed 's/.*{\([^{}]*\)}.*/\1/'))

PS_PICTURES=$(addsuffix .eps, $(PICTURES))
PDF_PICTURES=$(addsuffix .pdf, $(PICTURES))

## $(PICTURE_DB) keeps track of which pictures were actually created by
## this Makefile. In the clean target this database is used to remove them.
## You might have some manual work to do if you accidentially remove it.
PICTURE_DB = picture.db
PICTURE_DB_ADD = test -f $(PICTURE_DB) && grep -F "$@" $(PICTURE_DB) || echo "$@" >>$(PICTURE_DB)

PDFTK=/usr/bin/pdftk

## call pdflatex target if you prefer pdflatex over latex, dvips, ps2pdf

all: paper

paper: $(MAIN).tex $(TEXFILES) $(PDF_PICTURES) $(BIBLIOGRAPHY)
	pdflatex $@ $<
ifneq ($(BIBLIOGRAPHY), )
	bibtex $@ && pdflatex $@ $< && pdflatex $@ $<
endif
	(test -f $(PDFTK) && $(PDFTK) $@.pdf output $@.pdf Acompress) || cp $@.pdf $(MAIN)_out.pdf

# all: pdflatex
# # all: $(MAIN).pdf
# # all: pdflatex $(MAIN).ps $(MAIN).pdf
# # all: $(MAIN).pdf

# ## Detection of changed '\cite'ations is a PITA. Any hints welcome.


.PHONY: $(MAIN).ps $(MAIN).pdf $(MAIN).dvi

$(MAIN).ps: $(MAIN).dvi
	dvips -z -P pdf -t letter -o $@ $<

$(MAIN).pdf: $(MAIN).ps
	ps2pdf -dSAFER -dNOPLATFONTS -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $< $@

## Detection of changed '\cite'ations is a PITA. Any hints welcome.
$(MAIN).dvi: $(MAIN).tex $(TEXFILES) $(PS_PICTURES) $(MAIN).bbl
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).oc
	latex $<
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).nc
	cmp $(MAIN).oc $(MAIN).nc || bibtex $(MAIN) && latex $< && latex $<

$(MAIN).bbl: $(BIBLIOGRAPHY)
	latex $(MAIN).tex
	bibtex $(MAIN).aux || true
	latex $(MAIN).tex

## unfortunately produces broken pictures, fallback to eps and eps2pdf
#%.pdf: %.dia
#	dia --export=$@ $<
#	$(PICTURE_DB_ADD)

%.eps: %.dia
	dia --export=$@ $<
	$(PICTURE_DB_ADD)

%.pdf: %.fig
	fig2dev -L pdf $< $@
	$(PICTURE_DB_ADD)

%.eps: %.fig
	fig2dev -L eps $< $@
	$(PICTURE_DB_ADD)

%.eps: %.jpg
	convert $< $@
	$(PICTURE_DB_ADD)

%.pdf: %.png
	convert $< $@
	$(PICTURE_DB_ADD)

%.pdf: %.svg
	inkscape --export-pdf=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.svg
	inkscape --export-eps=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.wmf
	wmf2eps --eps -o $@ $<
	$(PICTURE_DB_ADD)

# this rule requires the R script to plot to the correct file,
# relative to the Makefile!
%.eps: %.R
	R --no-save <$<
	test -f $@
	test $@ -nt $<

## This generic rule should be kept as the last one, so that
## native -> pdf generation takes precedence over native -> eps -> pdf
#%.pdf: %.eps
#	epstopdf --outfile=$@ $<
#	$(PICTURE_DB_ADD)

%.eps: %.pdf
	pdftops -eps $< $@
	$(PICTURE_DB_ADD)

clean:
	rm -f *.aux *.dvi *.log *.nav *.out \
		*.pdf *.ps *.snm *.toc *.bbl \
		*.blg *.oc *.nc
	rm -f $(shell test -f $(PICTURE_DB) && cat $(PICTURE_DB))
	rm -f $(PICTURE_DB)

report-pictures:
	@echo $(PICTURES)

